Multi-level tree based approach for interactive graph visualization with semantic zoom

Human subject studies that map-like visualizations are as good or better than standard node-link representations of graphs, in terms of task performance, memorization and recall of the underlying data, and engagement [SSKB14, SSKB15]. With this in mind, we propose the Zoomable Multi-Level Tree (ZMLT) algorithm for multi-level tree-based, map-like visualization of large graphs. We propose seven desirable properties that such visualization should maintain and an algorithm that accomplishes them. (1) The abstract trees represent the underlying graph appropriately at different level of details; (2) The embedded trees represent the underlying graph appropriately at different levels of details; (3) At every level of detail we show real vertices and real paths from the underlying graph; (4) If any node or edge appears in a given level, then they also appear in all deeper levels; (5) All nodes at the current level and higher levels are labeled and there are no label overlaps; (6) There are no edge crossings on any level; (7) The drawing area is proportional to the total area of the labels. This algorithm is implemented and we have a functional prototype for the interactive interface in a web browser.

==> direct.tex <==


\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/Last_layer_drawing_dot.pdf}
    \caption{sfdp}
    \label{fig:pipeline_block}
\end{figure}
\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/sfdp_zoom.png}
    \caption{sfdp zoom}
    \label{fig:pipeline_block}
\end{figure}







\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/Last_layer_cross_free_drawing_dot_mod.pdf}
    \caption{crossing remove}
    \label{fig:pipeline_block}
\end{figure}





\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T1.pdf}
    \caption{T1}
    \label{fig:pipeline_block}
\end{figure}


 
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T2.pdf}
    \caption{T2}
    \label{fig:pipeline_block}
\end{figure}


\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T3.pdf}
    \caption{T3}
    \label{fig:pipeline_block}
\end{figure}


\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T4.pdf}
    \caption{T4}
    \label{fig:pipeline_block}
\end{figure}



\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T5.pdf}
    \caption{T5}
    \label{fig:pipeline_block}
\end{figure}


\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T6.pdf}
    \caption{T6}
    \label{fig:pipeline_block}
\end{figure}


\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T7.pdf}
    \caption{T7}
    \label{fig:pipeline_block}
\end{figure}


\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{results/direct_approach/T8.pdf}
    \caption{T8}
    \label{fig:pipeline_block}
\end{figure}


==> direct2.tex <==
\section*{Appendix}
\subsection*{Direct Approach (pipeline1)}

\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T1.pdf}
    \caption{Layer 1 extracted from the layout given by Direct Approach}
    \label{fig:T1DirectApproach}
\end{figure}
 
 
\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T2.pdf}
    \caption{Layer 2 extracted from the layout given by Direct Approach}
    \label{fig:T2DirectApproach}
\end{figure}

 
\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T3.pdf}
    \caption{Layer 3 extracted from the layout given by Direct Approach}
    \label{fig:T3DirectApproach}
\end{figure}
 
\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T4.pdf}
    \caption{Layer 4 extracted from the layout given by Direct Approach}
    \label{fig:T4DirectApproach}
\end{figure}

 
\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T5.pdf}
    \caption{Layer 5 extracted from the layout given by Direct Approach}
    \label{fig:T5DirectApproach}
\end{figure}

 
\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T6.pdf}
    \caption{Layer 6 extracted from the layout given by Direct Approach}
    \label{fig:T6DirectApproach}
\end{figure}

 
\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T7.pdf}
    \caption{Layer 7 extracted from the layout given by Direct Approach}
    \label{fig:T7DirectApproach}
\end{figure}

 
\begin{figure} 
    \centering
    \includegraphics[width=1\textwidth]{fig/direct/T8.pdf}
    \caption{Layer 8 drawn by Direct Approach}
    \label{fig:T8DirectApproachA}
\end{figure}

 
% \begin{figure} 
%     \centering
%     \includegraphics[width=0.4\textwidth]{results/direct2/T8dotmap.pdf}
%     \caption{dir2}
%     \label{fig:pipeline_block}
% \end{figure}


==> proposal.tex <==
\section{Related Work}~\label{sec:related}
Prior related work %that is relevant here 
spans topics such as 
%to the computation and visualization MLGS graphs covers 
algorithms for the layout of large graphs, %(where just one large layout is produced), 
algorithms for multi-level visualization of large graphs, overlap removal and topology preservation, and Steiner trees.

\paragraph{Large Graph Visualization:} Most graph layout algorithms use either a force-directed~\cite{eades1984heuristic,fruchterman1991graph} or a stress model~\cite{brandes2007eigensolver,koren2002ace} and provide a single static drawing.
%spring-electrical model or the stress model. The former (also known as force-directed method) starts with a random layout, the combined
%attractive and repulsive forces for each node are computed, and the nodes are moved along
%the direction of the force, until the layout stabilizes~\cite{Eades+1984a,Fruchterman_Reingold_1991}.
The force-directed model works well for small graphs, but does not scale for large networks. Speedup techniques employ a multi-scale variant~\cite{hh-msadg-99,GGK04} or use parallel computation as in VxOrd~\cite{DWB01,bkk-mbs-05}. 
%where a sequence of progressively coarser graphs is extracted from the underlying graph, followed by a sequence of progressively finer layouts, ending with a layout for the entire graph ~\cite{gk-grip-00,hh-msadg-99,harelkoren02,GGK04}
GraphViz~\cite{ellson2001graphviz} uses a multi-scale force-directed method and the SFDP algorithm~\cite{hu2005efficient} that combines the multi-scale approach with a fast $n$-body simulation~\cite{Barnes86a}. 
%The stress model assumes that there are springs connecting all pairs of nodes
%of the graph, with ideal spring length equal to the predefined edge weight.
Stress minimization was introduced in the more general setting of multidimensional scaling (MDS)~\cite{MDS} and has been used to draw graphs as early as 1980~\cite{seery1980designing}.
%What makes this particular stress function relevant to drawing large graphs is that it can be
Simple stress functions can be efficiently optimized by exploiting fast algebraic operations such as majorization.
%Specifically, the stress function can be globally minimized via majorization, which is guaranteed to converge.
Modifications to the stress model include the strain model (classical scaling)~\cite{torgerson1952},
PivotMDS~\cite{brandes2007eigensolver}, COAST~\cite{gansner2013coast}, and MaxEnt~\cite{gansner2013maxent}. 
%In the context of the strain model, a solution can be obtained by finding coordinates of nodes in a $k$-dimensional space, and then projecting back to 2D~\cite{harel2002graph,koren2002ace}.
Although these algorithms are fast
and produce good drawings of regular grid-like graphs, the results are not as good for dense graphs, or small-world graphs~\cite{brandes2009}. 
%;hence they are rarely used for visualizing large real-world networks.

Graph layout algorithms are provided in libraries such as GraphViz~\cite{ellson2001graphviz}, OGDF~\cite{chimani2011}, MSAGL~\cite{nachmanson2008}, and VTK~\cite{schroeder2000}, but they do not support interaction, navigation, and data manipulation. Visualization toolkits such as Prefuse~\cite{heer2005}, Tulip~\cite{auber2017tulip}, Gephi~\cite{bastian2009gephi}, and yEd~\cite{wiese2004yfiles} support visual graph manipulation, and while they can handle large graphs,
%While the utilized visualization methods scale well algorithmically,
their rendering often does not: even for graphs with a few thousand vertices, the amount of information rendered statically on the screen makes the visualization unusable.
%There are software applications designed for analyzing large networks optimized for specific domain applications, such as  %TouchGraph~\cite{tg}, NodeXL~\cite{hansen2010},


\paragraph{Multi-Level Visualization:} Research on interactive multi-level interfaces for exploring large graphs inculdes ASK-GraphView~\cite{abello2006}, topological fisheye views~\cite{ky-vlgcfg-04,GKN05}, and Grokker~\cite{rivadeneira21}. Software applications such as Pajek~\cite{de2011} for social networks, and Cytoscape~\cite{shannon2003} for biological data provide limited support for multi-level network visualization. Zinsmanier \textit{et al.}~\cite{zinsmaier2012interactive} proposed a technique to deal with visual clutter by adjusting the level of detail shown, using node aggregation and edge bundling. 

Most of these approaches rely on meta-vertices and meta-edges, which make interactions such as semantic zooming, searching, and navigation counter-intuitive,
as shown by Wojton \textit{et al.}~\cite{wojton2014sense} with a study involving more than a thousand youth and adult visitors to five science museums. This work confirms that people have difficulty reading graph layouts that use hierarchical cluster representations (via high-level meta-nodes and meta-edges) such as ``super-noding" and ``edge bundling."
%Also, well known graph drawing tools such as \textit{Graphviz}~\cite{ellson2001graphviz}%, or \textit{Gephi}~\cite{bastian2009gephi} do not provide such aggregation options when showing real nodes and edges is requested.
%On the other hand, recent work by Saket \textit{et al.}
Other studies that compare standard node-link representations with map-like visualizations show that map-like visualizations are superior in terms of task performance, memorization and engagement~\cite{saket2014node,saket2015map}. 
In this context, \textit{GraphMaps}~\cite{modal2018new} visualizes a graph using the map metaphor and provides different zoom levels, driven by an embedding of the entire underlying graph.
%revealing the structural properties of the graph and enables users to navigate the graph using zooming and panning the authors also develop an algorithmic framework to construct GraphMaps from any given mesh (generated from a 2D point set), and for any given number of zoom levels, presenting an algorithm for assigning nodes to zoom levels that minimizes the change in the number of nodes on visible on the screen while the user zooms in and out between the levels.This approach does not guarantee  the properties that we aim for; in particular edges are drawn as polygonal chains where maximal straight-line segments in the drawing are called rail and are shareable among edges.
 %\textit{Treevis.net}~\cite{shulz2011treevis} is a collection of tree representations in literature, the website version contains more than 300 techniques to draw trees organized by dimensionality (2D, 3D, or hybrid), edge representation (explicit, implicit, or hybrid), and node alignment (radial, axis-parallel, or free).
 GRAM~\cite{burd2018graph} also visualizes a graph using the map metaphor and provides different zoom levels but neither GraphMaps nor GRAM guarantees all six of our desirable properties. 
 For example, GRAM does not provide consistency or planarity. GRAM provides a button to show or hide the edges of the shown graph but the first option does not show the structure of the graph and the second one leads to the dreaded hairball; see Fig.~\ref{fig:Gramscreen}.
  %visualizes a graph in an interactive system using node clustering and map metaphor. The system shows node clustering and enables zooming, panning and navigation without any node overlap. GRAM grantees our multi-level properties real, persistent, overlap-free, compact but it does not ensure representative and planar properties. 
 %In fact, one of the challenges for the visualization of large graphs is the visual clutter produced by edges and labels (in case of labeled graphs).
 %
 %Another map-like visualization approach is \textit{GraphMaps}~\cite{modal2018new} a system that visualizes a graph using zoom levels revealing the structural properties of the graph and enables users to navigate the graph using zooming and panning  the authors also develop an algorithmic framework to construct GraphMaps from any given mesh (generated from a 2D point set), and for any given number of zoom levels, presenting an algorithm for assigning nodes to zoom levels that minimizes the change in the number of nodes on visible on the screen while the user zooms in and out between the levels. This approach does not guaratees the properties we aim in particular edges are drawn as polygonal chains where maximal straight-line segments in the drawing are called rail and are shareable among edges.
 
 \paragraph{Overlap Removal and Topology Preservation :} 
 In theory, vertices are usually treated as   point objects, but in practice, vertices are labeled and these labels must be shown in the layout. Overlapping labels is a major problem for most graph layout algorithms, and it severely affects the usability of the visualization. %associated and represented as their visualization labels may be another cause of visual clutter and degradation of readability: if labels overlap it could be not possible to read them.
 %
% Since most of the existing force directed algorithms place the vertices using physical model systems usually they do not have control on labels overlap in particular because, excluding some exceptions such as~\cite{chuang2004drawing,li2005using,wang1996generating}, they treat vertices as points without taking into account labels and size of the vertices. 
The standard approach to dealing with this problem is post-processing of the layout where node positions are perturbed to remove label overlaps. 

This usually results in significantly modified layout with increased stress, larger drawing area, and with the introduction of crossings even when the starting vertex configuration is crossings-free.
%have been proposed but the trade-off of getting an overlap-free drawing starting from a given drawing is to lose the characteristics of the input layout.
%
A simple solution to remove overlaps is  to scale the drawing until the labels no longer overlap. This approach works on every layout and is effective and straightforward, However, the area of the drawing may increase exponentially.
Marriott \textit{et al.}~\cite{marriott2003removing} proposed to scale the layout using different scaling factors for the $x$ and $y$ coordinates. This reduces the overall blowup in size but may result in poor aspect ratio.
Gansner and North~\cite{gansner1998improved},  Gansner and Hu~\cite{gansner2009efficient}, and Nachmanson \textit{et al.}~\cite{nachmanson2017node} describe overlap-removal techniques with better aspect ratio and modest additional area. However, none of these approaches, except the simplest scaling one can guarantee that no crossings are added when starting with a crossings-free input. 
%have been proposed by use Voronoi diagram for the graph and move the vertices in its cells, then edges are drawn as smooth curves to avoid label-edge overlaps. 
%A straight-line approach is the \textit{PRISM} algorithm proposed by  whose goal is to remove overlaps while preserving the shape of the initial layout by maintaining the proximity relations. This technique sets up a rigid ``scaffolding'' structure so that while vertices can move around their relative positions are maintained.
%Maintaining the original layout is an important factor as pointed out by Nachmanson \textit{et al.}~\cite{nachmanson2017node} who proposed \textit{GTree} an algorithm that  iteratively builds a Minimum Spanning Tree on a Delaunay triangulation of the node centers and removes the node overlaps by “growing” the tree. The goal of this algorithm is to keep the layout similar to the original one, but still does not guarantee to preserve the initial number of crossings. The authors of GTree show that this algorithm is faster than the  best performing algorithms, such as PRISM.
%These techniques are efficient concerning the overlap removal but they do not take into account the planarity or, more in general, the number of crossings of the input layout. Thus although these algorithms may improve the readability of the labels can reduce that given by planarity or a desired number of crossings. 
%

Post-processing a layout while preserving the topology of the input layout is a difficult task.  \textit{Pred}~\cite{bertault1999force} is a post-processing force directed algorithm applied on a given layout that aims to improve layout quality metrics while preserving the number of crossings. 
%, using three forces node-to-node repulsion force edge attractive force, edge-to-node repulsion force.
\textit{Impred}~\cite{simonetto2011impred} is an improved version that speeds-up the force computation and provides better results. This algorithm is not designed to remove the node overlaps but, with some appropriate modifications described in Section~\ref{se:removeoverlap}, it can be used for that purpose, while ensuring that the number of crossings remains unchanged. %changing the number of crossings that in our case will be planar.


\paragraph{Steiner Trees:}
The classic Steiner tree problem is one of Karp's  original 21 NP-Complete problems~\cite{karp1972}. A polynomial time approximation scheme exists if the underlying graph is planar~\cite{borradaile2007}, but not for general graphs~\cite{chlebik2008}.
More importantly, both the Steiner tree and metric Steiner tree (when edge weights satisfy the triangle inequality) can be efficiently approximated within a factor of $\ln 4 + e < 1.39$~\cite{byrka2010}. %The bottleneck Steiner tree, where the optimization is over the heaviest edge in the tree (rather than the sum of edges in the tree), can be solved exactly in polynomial time~\cite{sarrafzadeh1992}, although the $k$-bottleneck variant (restricting the number of Steiner vertices) remains NP-hard~\cite{abu2011}. 
In the vertex-weighted Steiner tree problem, the cost of the tree is determined by the weights of the vertices  included in the solution (rather than the weights of the edges). The problem is NP-hard~\cite{moss2007} but can be approximated within a logarithmic factor~\cite{guha1999}.
%
The classical Stainer tree problem has been also studied (using other terminology) in its multi-level version where the terminals appear on ``levels” and must be connected by edges of appropriate levels~\cite{ahmed2018multilevel,Balakrishnan1994ModelingAH,1288137,Chuzhoy:2008:AND:1361192.1361200,doi:10.1287/ijoc.8.3.202} while the multi-level version of the vertex-weighted Stainer tree has been studied in~\cite{darabi2018approximation}.
%
Since in this work we focus on the layout of trees a rich exposition of tree representations in literature is given by \textit{Treevis.net}~\cite{shulz2011treevis} a the website containing more than 300 techniques to draw trees organized by dimensionality (2D, 3D, or hybrid), edge representation (explicit, implicit, or hybrid), and node alignment (radial, axis-parallel, or free).
